Taming Mambas for Voxel Level 3D Medical Image Segmentation

Recently, the field of 3D medical segmentation has been dominated by deep learning models employing Convolutional Neural Networks (CNNs) and Transformer-based architectures, each with their distinctive strengths and limitations. CNNs are constrained by a local receptive field, whereas transformers are hindered by their substantial memory requirements as well as they data hungriness, making them not ideal for processing 3D medical volumes at a fine-grained level. For these reasons, fully convolutional neural networks, as nnUNet, still dominate the scene when segmenting medical structures in 3D large medical volumes. Despite numerous advancements towards developing transformer variants with subquadratic time and memory complexity, these models still fall short in content-based reasoning. A recent breakthrough is Mamba, a Recurrent Neural Network (RNN) based on State Space Models (SSMs) outperforming Transformers in many long-context tasks (million-length sequences) on famous natural language processing and genomic benchmarks while keeping a linear complexity.

==> figures/bidir3dmamba.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.4\textwidth]{imgs/Bidir3DMamba}
    \caption{Depiction of our Bidirectional 3D Mamba Layer. The input is a batch of 3D volumes in the form (B, H, W, D, C), where B is the batch size, H, W, D are the spatial dimensions (height, width, depth), and C is the number of channels. All purple blocks refer to torch methods. The spatial dimension are flattened to get a 1D sequence (B, L, C) where $L = H*W*D$, and a backward version of the sequence is produced by the \texttt{.flip()}. Both forward and backward sequence are inferred through two different Mamba layers then summed after the backward is flipped back to the original order. A final reshape brigs the shape back to (B, H, W, D, C).}
\label{fig:bidir3dmamba}
\end{figure}

==> figures/dataset.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table: Table datasets                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\caption{Summary description of the ToothFairy dataset.}
\centering
\small
\begin{tabular}{c c c c c}
\toprule
\multirow{2}{*}{\vspace{-5pt}\textbf{Dataset}} &
\multirow{2}{*}{\vspace{-5pt}\textbf{Split}} &
\multirow{2}{*}{\vspace{-5pt}\textbf{Volumes}} &
\multicolumn{2}{c}{\textbf{Annotations}} \\
\cmidrule(lr){4-5}
  
& & &
\textbf{2D} & 
\textbf{3D} \\
  \midrule

\multirowcell{3}{Primary} & Training & 153 & \cmark & \cmark  \\
 	           & Validation & 8 & \cmark & \cmark  \\
 	           & Testing & 15 & \cmark & \cmark \\
\midrule
                Secondary & Training &	290 & \cmark &	\xmark  \\	


\bottomrule
\end{tabular}


\label{tab:dataset}
\vspace{-10pt}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> figures/gt_and_preds.tex <==
% \begin{figure*}[hb]
%     \centering
%     \begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
%         \includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/acdc/data.png} & \hspace{1pt} & \includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/acdc/gt.png} & \hspace{1pt} & \includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/acdc/seg.png} & \hspace{1pt} & \includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/acdc/pan.png} & \hspace{1pt} & \includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/acdc/skip.png} \\
%         \subfloat[]{\includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/brain/data.png}} & \hspace{1pt} &
%         \subfloat[]{\includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/brain/gt.png}} & \hspace{1pt} & \subfloat[]{\includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/brain/seg.png}} & \hspace{1pt} & \subfloat[]{\includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/brain/pan.png}} & \hspace{1pt} &
%         \subfloat[]{\includegraphics[width=0.19\textwidth,valign=c]{imgs/gt_and_preds/brain/skip.png}}
%     \end{tabular}
%     \caption{Example of predictions of our proposed networks. Column (a) corresponds to the input image, column (b) corresponds to the ground truth, column (c) corresponds to \SegMamba{}, column (d) corresponds to \PanSegMamba{}, column (e) corresponds to \SegMambaSkip{}.
%     }
%     \label{fig:gt_and_preds}
% \end{figure*}

==> figures/model.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.49\textwidth]{matap}
    \caption{Proposed module integrated in the standard 3D \unet{} architecture. A detailed visualization of our module is reported in \cref{fig:matap_module}.}
    \vspace{-10pt}
\label{fig:model}
\end{figure}

==> figures/patch-training.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.5\textwidth]{imgs/Patch-based-learning-unet}
    \caption{Visualization of a patch-based training. From the original volume, depicted in blue, a sub-volume is extracted and fed into the network. The output, depicted in green, is then placed in the same position where the patch has been extracted.}
\label{fig:multidir3dmamba}
\end{figure}

==> tables/results_KiTS23.tex <==
\begin{table*}[tb]
  \setlength{\tabcolsep}{6pt}
  \centering
  \caption{Results on the KiTS23 dataset. Our proposals are marked with $\dagger$.The evaluation metric is the DSC (\%). Best results are in bold while second best are underlined. *5-folds cross validation}
  \begin{tabular}{l
  >{\columncolor{PrimaryColumnColor}}S[table-auto-round,table-format=2.2]
  c
  >{\columncolor{PrimaryColumnColor}}S[table-auto-round,table-format=2.2]
  c
  }
    \toprule
    \textbf{Methods} & \cellcolor{SecondaryColumnColor} \textbf{Average} & \textbf{Kidney} & \cellcolor{SecondaryColumnColor} \textbf{Tumor}   & \textbf{Cyst}    \\
    \midrule
    TransUNet \cite{chen2021transunet}           &         &  &   & \\
    TransBTS \cite{wang2021transbts} \\ 
    CoTr \cite{xie2021cotr} \\
    
    UNETR \cite{hatamizadeh2022unetr}  \\
    UNETR++ \cite{Shaker2024}         \\
    
    UMambaBot  \cite{Ma2024}                     &  86.22* &  &   &  \\
    UMambaEnc  \cite{Ma2024}                     &  86.34* &  &   &  \\
    Altro Mamba TODO \\
    
    MedNeXt (S/B/M) \cite{Roy2023}               &         &  &   &  \\

    nnUNet \cite{isensee2021nnu}  & 86.04*   & &  &  \\
    nnFormer \cite{zhou2023nnformer}    & \textbf{92.06}*   &  & &  \\
    nnUNet ResEnc M  \cite{Isensee2024}          &  86.79* &  &   &  \\
    nnUNet ResEnc L  \cite{Isensee2024}          &  88.17* &  &   &  \\

    \midrule
    \SegMamba{}$\dagger$  & & & & \\
    \PanSegMamba{}$\dagger$  &  &  &  &  \\
    \SegMambaSkip{}$\dagger$ &  &  &  &  \\
    % \PanSegMamba{}_pos & 
    \bottomrule
  \end{tabular}
  \label{tab:acdc_results}
\end{table*}
